TOAST: Fast and scalable auto-partitioning based on principled static analysis

Partitioning large machine learning models across distributed accelerator systems is a complex process, requiring a series of interdependent decisions that are further complicated by internal sharding ambiguities. Consequently, existing auto-partitioners often suffer from out-of-memory errors or are prohibitively slow when exploring the exponentially large space of possible partitionings. To mitigate this, they artificially restrict the search space, but this approach frequently yields infeasible solutions that violate device memory constraints or lead to sub-optimal performance. We propose a system that combines a novel static compiler analysis with a Monte Carlo Tree Search. Our analysis constructs an efficient decision space by identifying (i) tensor dimensions requiring identical sharding, and (ii) partitioning "conflicts" that require resolution. Our system significantly outperforms state-of-the-art industrial methods across diverse hardware platforms and model architectures, discovering previously unknown, superior solutions, and the process is fully automated even for complex and large models.

==> sections/arch.tex <==
\subsection{System architecture} 
The automatic partitioner we present in this paper is a frontend (i.e., JAX~\cite{jax2018github}, PyTorch~\cite{pytorch2019}) and backend agnostic (e.g., XLA\cite{xla}). Instead, it operates over an array program representation -- StableHLO~\cite{stablehlo},
which is an MLIR dialect \cite{mlir2020} that frontends can compile to, and backend compilers can compile and execute on a 
variety of hardware platforms.
% StableHLO provides the types and shapes of the tensors and the operations in the program.
% A common entry point for our users is JAX\cite{jax2018github} which by default lowers to StableHLO during the compilation process.
% % The users enable the auto-partitioning process by enabling a flag that indicates they want the partitioner to make decisions on the module -- currently we only support fully unpartitioned module - but it is trivial to support partially partitioned module (mainly we just apply the same workflow as unpartitioned module then apply the users' manual partitioning decisions on top of our analysis, before any of \toast{}'s processes kick-in). 
% % in the details of the dialect are peer-reviewed and published in a separate work~\cite{anon} (anonymized for submission). 
% These details are more of a practical concerns of where \toast{} sits in the stack and how users interact with it - we will focus the rest of the paper on the two main components of \toast{}: The named dimension analysis (\Cref{sec:NDA}) and \toast{} (\Cref{sec:toast}). 

\begin{figure}
    \centering
    % https://docs.google.com/drawings/d/13YSxJAOIGtl6MHl7_a-e_uFYhIYAcaooxJkxzuTD4Ag/edit?resourcekey=0-o5bQXUTYdAg6GxKMdY1f3g
    \includegraphics[width=\linewidth]{figures/toast-arch-simpl.pdf}
    \caption{\label{fig:arch}\toast{} overall system architecture.}
\end{figure}

\Cref{fig:arch} tracks the various components of \toast{} from StabelHLO to a final sharded module.
\begin{enumerate}
    \item First we apply user hints or invoke automatic-grouping heuristics~\dvytin{ref to section or prev discussion} to
    identify groups of parameters of the model that should be sharded the same.(\Cref{sec:grouping}).

    \item NDA is invoked taking into account the previous groups, to identify named dimension in the module, identify compatible
    conflict groups, and create the space of sharding actions (as different orders of iterating through conflict groups).
    % \item 
    % The named dimension analysis is invoked to identify unique dimensions in the module and create the space of sharding actions, \Cref{sec:NDA}.
    % \item A powerful unification pass through the unique names unifies the names according to a recursive function that reduces the number of unique names based on mathematical equivalence rules, which reduces the space of sharding decisions a user or search algorithm need to make \Cref{sec:NDA:version-2}.
    % \item From the remaining uniquely identified dimension, the NDA applies conflict compatibility analysis to identify conflicts that otherwise a propagation system would not know how to resolve and expose handlers for these action, \Cref{sec:NDA:handling-conflicts}.
    \item \toast{} runs iteratively until budget runs out, in each iteration it invokes a Monte Carlo Tree Search (MCTS) co-routine, across all available threads, \Cref{sec:toast}. The MCTS goal is to find a sequence of sharding decisions that improves the cost model signal, after each decision it queries the dataflow analysis \dvytin{Which dataflow analysis...?} to identify the actions that are still available to explore, \Cref{sec:action_design}. 
    \item Finally, the sequence of sharding decisions passed to a cost model that estimates the runtime and peak memory performance of the partitioned module and provide a signal back to the MCTS, \Cref{sec:cost_model}.
\end{enumerate}
The final output is a partitioned module that aims to improve on the unpartitioned module. 


